Generalized Cross-domain Multi-label Few-shot Learning for Chest X-rays

Real-world application of chest X-ray abnormality classification requires dealing with several challenges: (i) limited training data; (ii) training and evaluation sets that are derived from different domains; and (iii) classes that appear during training may have partial overlap with classes of interest during evaluation. To address these challenges, we present an integrated framework called Generalized Cross-Domain Multi-Label Few-Shot Learning (GenCDML-FSL). The framework supports overlap in classes during training and evaluation, cross-domain transfer, adopts meta-learning to learn using few training samples, and assumes each chest X-ray image is either normal or associated with one or more abnormalities. Furthermore, we propose Generalized Episodic Training (GenET), a training strategy that equips models to operate with multiple challenges observed in the GenCDML-FSL scenario. Comparisons with well-established methods such as transfer learning, hybrid transfer learning, and multi-label meta-learning on multiple datasets show the superiority of our approach.

==> tables/F1_MACE_thres_oracle.tex <==
\begin{table*}
\centering
\scriptsize
\begin{tabular}{@{}ccccccc@{}}
\toprule
\textbf{Method} & \textbf{F1-Score}         & \textbf{MACE}        & \textbf{F1-Score}         & \textbf{MACE}        & \textbf{F1-Score}      & \textbf{MACE}      \\ \midrule
                & \multicolumn{2}{c}{NIH → CheXpert}   & \multicolumn{2}{c}{NIH → PadChest}   & \multicolumn{2}{c}{NIH → MIMIC} \\ \midrule
TL    &                 &  &  &                 &  &        \\
HTL   &                 &  &  &                 &  &        \\
GenET & \textbf{0.5803} &  &  & \textbf{0.8898} &  & 0.4144 \\ \midrule
                & \multicolumn{2}{c}{MIMIC → CheXpert} & \multicolumn{2}{c}{MIMIC → PadChest} & \multicolumn{2}{c}{MIMIC → NIH} \\ \midrule
TL    &                 &  &  &                 &  &        \\
HTL   &                 &  &  &                 &  &        \\
GenET & \textbf{0.5733} &  &  & \textbf{0.8922} &  & 0.4074 \\ \bottomrule
\end{tabular}
\caption{F1 Scores and MACE of TL, HTL and GenET on CheXpert, PadChest, and MIMIC (NIH) datasets following training on the NIH (MIMIC) dataset with threshold 0.5. MMAML is multi-label MAML where fine-tuning set is absent in training episode, and there is a complete overlap between the support and query classes. }
\label{tab:test-th}
\end{table*}
